Era3D: High-Resolution Multiview Diffusion using Efficient Row-wise Attention

In this paper, we introduce Era3D, a novel multiview diffusion method that generates high-resolution multiview images from a single-view image. Despite significant advancements in multiview generation, existing methods still suffer from camera prior mismatch, inefficacy, and low resolution, resulting in poor-quality multiview images. Specifically, these methods assume that the input images should comply with a predefined camera type, e.g. a perspective camera with a fixed focal length, leading to distorted shapes when the assumption fails. Moreover, the full-image or dense multiview attention they employ leads to an exponential explosion of computational complexity as image resolution increases, resulting in prohibitively expensive training costs. To bridge the gap between assumption and reality, Era3D first proposes a diffusion-based camera prediction module to estimate the focal length and elevation of the input image, which allows our method to generate images without shape distortions. Furthermore, a simple but efficient attention layer, named row-wise attention, is used to enforce epipolar priors in the multiview diffusion, facilitating efficient cross-view information fusion. Consequently, compared with state-of-the-art methods, Era3D generates high-quality multiview images with up to a 512*512 resolution while reducing computation complexity by 12x times. Comprehensive experiments demonstrate that Era3D can reconstruct high-quality and detailed 3D meshes from diverse single-view input images, significantly outperforming baseline multiview diffusion methods. Project page: https://penghtyx.github.io/Era3D/.

==> arxiv_abstract.tex <==
  In this paper, we introduce \textbf{\methodname}, a novel multiview diffusion method that generates high-resolution multiview images from a single-view image. 
  Despite significant advancements in multiview generation,
  % existing methods like Wonder3D and SyncDreamer,  
  existing methods still suffer from camera prior mismatch, inefficacy, and low resolution, resulting in poor-quality multiview images.
  % so they barely generate high-quality multiview images. 
  Specifically, these methods assume that the input images should comply with a predefined camera type, e.g. a perspective camera with a fixed focal length, leading to distorted shapes when the assumption fails.
  % First, these methods assume a  of the input image, leading to distorted shapes when the real intrinsic differs. 
  Moreover, the full-image or dense multiview attention they employ leads to an exponential explosion of computational complexity as image resolution increases, resulting in prohibitively expensive training costs.
  % making model training computationally expensive. 
  % thus yielding unaffordable computational consumption for model training.
  % the multiview consistency is achieved by dense multiview attention, which is inefficient for high-resolution training due to high computation complexity. 
  To bridge the gap between assumption and reality, \methodname first proposes a diffusion-based camera prediction module to estimate the focal length and elevation of the input image, which allows our method to generate images without shape distortions.
  % and incorporating it into the diffusion process. This design allows the model to predict accurate camera pose, and further generate multi-views in canonical orthogonal camera settings without any camera prior.
  % \methodname addresses the above problems by proposing a new regression and condition scheme to generate images in the canonical camera settings while allowing input images to have arbitrary intrinsic.
  Furthermore, a simple but efficient attention layer, named row-wise attention, is used to enforce epipolar priors in the multiview diffusion, facilitating efficient cross-view information fusion.
  Consequently, compared with state-of-the-art methods, \methodname generates high-quality multiview images with up to a 512$\times$512 resolution while reducing computation complexity by 12x times. Comprehensive experiments demonstrate that \methodname can reconstruct high-quality and detailed 3D meshes from diverse single-view input images, significantly outperforming baseline multiview diffusion methods. Project page: \textbf{\url{https://penghtyx.github.io/Era3D/}}.

==> arxiv_introduction.tex <==
\begin{figure}
\centering
\includegraphics[width=\textwidth, bb=0 0 800 600]{figures/teaser.jpg}
    \footnotesize \leftline{~~~Input images~~\qquad\quad\quad~Generated images~~~~\qquad\qquad\qquad~Generated normal maps~~~~\quad~~Output mesh}
    \vspace{-10pt}
    \caption{Given single-view image with arbitrary intrinsic and viewpoints, \methodname can generate high-quality multiview images with a resolution of $512\times512$ on the orthogonal camera setting, which can be used in mesh reconstruction by NeuS~\cite{wang2021neus}.}
    \label{fig:teaser}
\end{figure}

3D reconstruction from single-view images is an essential task in computer vision and graphics due to its potential applications in game design, virtual reality, and robotics.
% which enables us to generate 3D assets for different downstream applications. 
Early research~\cite{park2019deepsdf, peng2020convolutional, saito2019pifu, zheng2023learning} mainly relies on direct 3D regression on voxels~\cite{niessner2013real, sun2022direct, cheng2023sdfusion}, which often leads to oversmoothed results and has difficulty in generalizing to real-world unseen objects due to limited 3D training data~\cite{chang2015shapenet}. 
Recently, diffusion models (DMs)~\cite{ho2020denoising,ldm} show strong generation ability on image or video synthesis by training on extremely large-scale datasets. These diffusion models are promising tools for single-view 3D reconstruction because it is possible to generate novel-view images from the given image to enable 3D reconstruction.
% In recent two years, generative AI has achieved significant breakthroughs in diverse domains, including image~\cite{}, video~\cite{} and audio~\cite{}. However, 3D content generation remains challenging due to the space ambiguity and the lack of training data. 

% single view 3D reconstruction is useful
% A simple review of single view reconstruction: SDS to multiview diffusion
% two challenges:
% how we address these two challenges
% results

To utilize image DMs for single-view 3D reconstruction, a pioneer work DreamFusion~\cite{poole2022dreamfusion} tries to distill a 3D representation like NeRF~\cite{mildenhall2021nerf} or Gaussian Splatting~\cite{tang2023dreamgaussian} from a 2D image diffusion by a Score Distillation Sampling (SDS) loss and many follow-up works improve the distillation-based methods in quality~\cite{wang2024prolificdreamer} and efficiency~\cite{tang2023dreamgaussian}. However, these methods suffer from unstable convergence and degenerated quality. Alternatively, recent works such as MVDream~\cite{shi2023mvdream}, SyncDreamer~\cite{liu2023syncdreamer}, Wonder3D~\cite{long2023wonder3d} and Zero123++~\cite{shi2023zero123++} explicitly generate multiview images by multiview diffusion~\cite{tang2023MVDiffusion,liu2023syncdreamer} and then reconstruct 3D models from the generated images by neural reconstruction methods~\cite{wang2021neus} or large reconstruction models (LRMs)~\cite{hong2023lrm,li2023instant3d}. Explicitly generating multiview images makes these methods more controllable and efficient than SDS methods and thus is more popular in the single-view 3D reconstruction task.  

Despite impressive advancements in multiview diffusion methods~\cite{shi2023mvdream,long2023wonder3d,liu2023syncdreamer, sargent2023zeronvs, liu2023zero123, liu2023one2345, wang2023imagedream, tang2023MVDiffusion, tang2023MVDiffusion, tang2024mvdiffusion++, xu2023dmv3d, li2023instant3d}, efficiently generating novel-view images for high-quality 3D reconstruction remains an open challenge. There are three noticeable challenges in the current multiview diffusion methods.
(1) \textbf{Inconsistent predefined camera type}. Most multiview diffusion methods assume that the input images are captured by a camera with a predefined focal length. This leads to unwanted distortions when input images are captured by cameras with different camera types or intrinsics, as exemplified in Fig.~\ref{fig:distortion} (e.g., Wonder3D's assumption of an orthogonal camera leads to distorted meshes when the input image is captured by a perspective camera with a small focal length). 
(2) \textbf{Inefficiency of multiview diffusion}. Multiview diffusion methods usually rely on multiview attention layers to exchange information among different views to generate multiview-consistent images. 
However, these multiview attention layers are usually implemented by extending the self-attention in Stable Diffusion~\cite{rombach2021stablediffusion} to all multiview images, which is called dense multiview attention in Fig.\ref{fig:attention_comp}(a) and results in a significant increase in computation complexity and memory consumption. 
(3) \textbf{Low resolution of generated images}. The limitation above restricts most existing multiview diffusion models to resolutions of $256\times 256$, preventing them from reconstructing detailed meshes. Addressing these above challenges is crucial for developing practical and scalable multiview diffusion methods.

\begin{figure}
    \scriptsize
 
    \centering
    \includegraphics[width=\textwidth, bb=0 0 850 200]{figures/attention_comp.jpg}
    \leftline{~\quad~~(a) Dense Attention~\quad~{(b) General Camera Setting~\quad~~(c) Epipolar Attention~\quad~(d) Canonical Camera Setting~~~~~(e) Row-wise Attention}}
    \leftline{~~\qquad\quad~~$O(N^2S^4)$~~\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad~$O(N^2S^2K)$~\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad~$O(N^2S^3)$}
    \caption{Different types of multiview attention layers. (\textbf{a}) In a dense multiview attention layer, all feature vectors of multiview images are fed into an attention block.
    For a general camera setting (\textbf{b}) with arbitrary viewpoints and intrinsics, utilizing epipolar constraint to construct an epipolar attention (\textbf{c}) needs to correlate the features on the epipolar line. This means that we need to sample $K$ points along each epipolar line to compute such an attention layer. In our canonical camera setting (\textbf{d}) with orthogonal cameras and viewpoints on an elevation of 0$^{\circ}$, epipolar lines align with the row of the images across different views (\textbf{e}), which eliminates the need to resample epipolar line to compute epipolar attention. We assume the latent feature map has a resolution of $H\times W$ and $H=W=S$. In such a $N$-view camera system, row-wise attention reduces the computational complexity to $O(N^2S^3)$.
    % epipolar attention can be efficiently implemented using a row-wise attention layer, which reduces the computational complexity to $O(N^2S^3)$.
    }
    \vspace{-10pt}
    \label{fig:attention_comp}
\end{figure}

In this paper, we introduce \methodname, a novel multiview diffusion method that efficiently generates high-resolution (512$\times$512) consistent-multiview images for single-view 3D reconstruction. Unlike existing methods, \methodname allows images of commonly used camera types as inputs while mitigating the unwanted distortion brought by different camera models. To this end, we employ a unique approach: using different camera models for input images and the generated ones for training, meaning that the input images are allowed to have arbitrary focal lengths and elevations while generated images are with orthogonal cameras and fixed viewpoints of 0$^\circ$ elevations. 
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \vspace{-10pt}
\includegraphics[width=0.45\textwidth]{figures/distortion.jpg}
\footnotesize\leftline{~~~~\quad~~~~Input~\quad~Generated images and mesh}
    \caption{(top) Perspective input images for Wonder3D produce extreme distortion in the generation. (bottom) \methodname can handle images of commonly used intrinsics.}
    \label{fig:distortion}
    \vspace{-10pt}
\end{wrapfigure}
However, this requires DMs to implicitly infer and rectify the focal lengths and viewpoints of input images in the generation process, which is a challenging task and degenerates the generation quality. To overcome this challenge and improve generation quality, we propose a novel regression and condition scheme and utilize the low-level feature maps of UNet at each denoising step to predict camera information of input images. We find that such a regression and condition scheme facilitates much more accurate camera pose prediction than existing methods~\cite{liu2023one2345} and leads to more details in the generation. 
% we further propose a regression and condition scheme that greatly reduces the difficulty in guessing the focal lengths and viewpoints of input images.
As shown in Fig.~\ref{fig:distortion}, \methodname successfully avoids the above distortion problem brought by the different camera types and focal lengths. 

Moreover, drawing inspiration from epipolar attention~\cite{tseng2023consistent}, \methodname enables efficient training for high-resolution multiview generation by introducing a novel row-wise multiview attention. Epipolar constraint can be utilized to constrain the attention regions across views and thus improve attention efficiency. 
However, directly applying such epipolar attention~\cite{tseng2023consistent} for a general camera setting (Fig.~\ref{fig:attention_comp}(b)) is still memory and computationally inefficient because we have to sample multiple points on epipolar lines for attention. This requires us to construct a 3D grid of features in the view frustums for multiview images, which is too slow and memory-consuming.  
In contrast, since \methodname generates images with orthogonal cameras on viewpoints of $0^\circ$, we find that epipolar lines in our camera setting are aligned with rows of images across different views~(Fig.~\ref{fig:attention_comp}(d)), which enables us to propose an efficient row-wise attention layer.
Compared with dense multiview attention, row-wise attention significantly reduces memory consumption ($35.32$GB v.s. $1.66$GB), and the computation complexity ($220.41$ms v.s. $2.23$ms) of multiview attention~(Fig.~\ref{fig:attention_comp}(e)). 
%Compared with dense multiview attention, row-wise attention significantly reduces memory consumption (35.32 v.s. 1.66GB), and the computation complexity (220.41 v.s. 2.23ms) of multiview attention~(Fig.~\ref{fig:attention_comp}(e)). 
Even with Xformers~\cite{xFormers2022}, an accelerating library for attention, the efficiency of row-wise attention still outperforms existing methods by approximately twelve-fold as evident in Tab.~\ref{tab:abla_rowwise}. Consequently, the proposed row-wise attention allows us to easily scale \methodname to a high resolution of 512$\times$512 to reconstruct more detailed 3D meshes.  
% \methodname enables an efficient multiview attention mechanism by utilizing epipolar lines to constrain the attention regions. Directly applying such an epipolar attention layer~\cite{tseng2023consistent} is still very memory and computation inefficient on general perspective cameras because we have to sample multiple points on epipolar lines and conduct attention layers on these sample points. This will require us to construct a 3D grid of features in the view frustum for multiview attention layers, which is too slow and memory-consuming. Since \methodname utilizes the orthogonal cameras on predefined canonical viewpoints, we find that the epipolar lines are just the rows of the generated images, which enables us to propose an efficient row-wise attention layer to greatly reduce the computation in the multiview attention layers. This enables us to easily scale \methodname to a high resolution of 512$\times$512 to reconstruct more details on 3D meshes.

% In the paper, we claim that pretrained T2I models have the ability to perceive the perspective distortion and observation view of in-the-wild images and convert it to the canonical orthogonal space (COS). Therefore, we propose a end-to-end fine-tuning framework, \methodname, to generate high-quality and consistent multiview images for 3D creation. Specifically, to predict the camera paramters, we design Elevation and Focal Regressor (EFReg), which takes as input the lowest level features in the UNet and output the elevation and focal lens related 2-Dimension vector. Then, we use the vector as additional condition to guide the denoising process. This novel design provides strong prior for SD to convert the viewport to the COS. To further improve generation quality and remain the cross view consistency, inspired by the epipolar theory, we propose Row-wise MVdiffusion, an efficient and 3D-aware multiview attention block. This design greatly reduces the redundant attention computation between multi views and allows for high resolution training.

Overall, our main contributions are summarized as follows: (1) \methodname is the first method that tries to solve the distortion artifacts brought by the inconsistent camera intrinsic in 3D generation; (2) we design a novel regression and condition scheme to enable diffusion models to take images of arbitrary cameras as inputs while outputting the orthogonal images on the canonical camera setting; (3) we propose row-wise multiview attention, an efficient attention layer for high-resolution multiview image generation; (4) our method achieve state-of-the-art performance for single-view 3D generation~\cite{deitke2023objaverse}.

